Potential gain as a centrality measure

Navigability is a distinctive features of graphs associated with artificial or natural systems whose primary goal is the transportation of information or goods. We say that a graph $\mathcal{G}$ is navigable when an agent is able to efficiently reach any target node in $\mathcal{G}$ by means of local routing decisions. In a social network navigability translates to the ability of reaching an individual through personal contacts. Graph navigability is well-studied, but a fundamental question is still open: why are some individuals more likely than others to be reached via short, friend-of-a-friend, communication chains? In this article we answer the question above by proposing a novel centrality metric called the potential gain, which, in an informal sense, quantifies the easiness at which a target node can be reached. We define two variants of the potential gain, called the geometric and the exponential potential gain, and present fast algorithms to compute them. The geometric and the potential gain are the first instances of a novel class of composite centrality metrics, i.e., centrality metrics which combine the popularity of a node in $\mathcal{G}$ with its similarity to all other nodes. As shown in previous studies, popularity and similarity are two main criteria which regulate the way humans seek for information in large networks such as Wikipedia. We give a formal proof that the potential gain of a node is always equivalent to the product of its degree centrality (which captures popularity) and its Katz centrality (which captures similarity).

==> computation.tex <==
% --------------------------------------------------------------------------
\section{Methods for computing the Geometric and Exponential Potential Gain}
\label{sec:methods}

\blue{In this section we prove that our algorithm to calculate the geometric and the exponential potential gain is convergent, and we provide an upper bound on the rate of convergence.}

%This section \red{explores} the accuracy of our algorithms to calculate geometric and exponential potential gain.
Let $\mathbf{g}$ be the true value of the geometric potential gain and let $\mathbf{g}_k$ be the approximate value of geometric potential gain we would obtain by considering walks up to length $k$.
We wish to estimate:

\begin{equation}
\label{eqn:varepsilon-geometric}
\varepsilon_g(k) = \frac{\norm{\mathbf{g} - \mathbf{g}_k}}{\norm{\mathbf{g}}}
\end{equation}

\noindent
Analogously, the approximation error associated with the calculation of the exponential potential gain is given by

\begin{equation}
\label{eqn:varepsilon-exponential}
\varepsilon_e(k) = \frac{\norm{\mathbf{e} - \mathbf{e}_k}}{\norm{\mathbf{e}}}
\end{equation}

The evaluation of $\varepsilon_g(k)$ and $\varepsilon_e(k)$ requires us to evaluate the {\em norm} of some matrices; here we will rely on the $L_2$ {\em matrix norm} (also known as {\em the spectral norm}), which, in case of symmetric matrices coincides exactly with $\lambda_1$ \cite{heath2002scientific}. 

Since all matrix norms defined over a space of finite-dimension matrices are equivalent, our results generalize to other matrix norms; the only requirement is that the {\em sub-multiplicative property} holds, i.e., $\norm{\mathbf{X}\times \mathbf{Y}} \leq \norm{\mathbf{X}}\norm{\mathbf{Y}}$ for any pair of matrices $\mathbf{X}$ and $\mathbf{Y}$. 



% ---------------------------------------------------------------
\subsection{Rate of convergence for the geometric potential gain}
\label{sub:rate-convergence-geometric}

Regarding the assessment of $\varepsilon_g(k)$, we note that the source of error in approximating the geometric potential gain depends on the early stopping of the Neumann series, i.e., on the approximation:

\begin{equation}
\label{eqn:early-stopping-neuman}
\left(\mathbf{I} -\delta\mathbf{A}\right)^{-1} \simeq \mathbf{I} + \delta\mathbf{A} + \delta^2\mathbf{A}^2 + \ldots
\delta^k\mathbf{A}^k  
\end{equation}
 
\noindent
Now, if we set $\mathbf{S}_k = \sum_{i=0}^{k} \delta^i\mathbf{A}^i$, the error $\varepsilon_g(k)$ depends on:

\begin{dmath}
\left( \mathbf{I} -\delta\mathbf{A}\right)^{-1} - \mathbf{S}_k = \left(\delta\mathbf{A}\right)^k +
\left(\delta\mathbf{A}\right)^{k+1} + \ldots = \left(\delta\mathbf{A}\right)^k \times\left(\mathbf{I} + \delta\mathbf{A} + \ldots \right) =
 \left(\delta\mathbf{A}\right)^k\left( \mathbf{I} -\delta\mathbf{A}\right)^{-1} 
\end{dmath}

\noindent
%A well-known result \cite{young1981rate,higham2008functions} about the convergence of $\varepsilon_g(k)$ as $k \to \infty$ yields the following:
As $k \to \infty$ we obtain:

\begin{dmath}
\norm{\left( \mathbf{I} -\delta\mathbf{A}\right)^{-1} - \mathbf{S}_k}^{\frac{1}{k}} = \norm{\left(\delta\mathbf{A}\right)^k\left( \mathbf{I} -\delta\mathbf{A}\right)^{-1}}^{\frac{1}{k}} \leq
\norm{\delta^k\mathbf{A}^k}^{\frac{1}{k}}\norm{\left( \mathbf{I} -\delta\mathbf{A}\right)^{-1}}^{\frac{1}{k}}
\end{dmath}

Moreover, as $k \to +\infty$, $\norm{\delta^k\mathbf{A}^k}^{\frac{1}{k}}$ converges to $\lambda_1$ \cite{cvetkovic1997eigenspaces}.
This result, however, is rather weak as it does not give us a realistic estimation of the number of iterations that are required to assure that $\varepsilon_g(k) \le \varepsilon$, for any $\varepsilon > 0$.

A more refined estimation of the rate of convergence of $\varepsilon_g(k)$ that applies to the general case of square complex matrices is due to Young \cite{young1981rate}, who provides a bound of the form $O(\lambda_1^{k-n} k^n)$; it depends on $\lambda_1$, on the number \textit{k} of iterations and, finally, on the size $n$ of $\mathbf{A}$.

Since we are dealing with symmetric matrices, we can derive simpler bounds that are independent of the matrix size, as proved below.

\begin{theorem}
\label{the:convergence-geometric}
Let $\G$ be a graph with adjacency matrix $\A$ and let $\lambda_1$ be its spectral radius; 
also let $\delta \in \left(0, \lambda_1^{-1}\right)$. 
Then $\varepsilon_g(k) \to 0$ with convergence rate $\left(\delta\lambda_1\right)^k$.
\end{theorem}


\begin{proof}
Recall that matrix $\mathbf{A}$ is square and symmetric thus it admits the following eigendecomposition

\[
\mathbf{A} = \mathbf{D}^{-1} \times \mathbf{\Lambda} \times \mathbf{D}
\]

where $\mathbf{\Lambda}$ is a diagonal matrix storing the eigenvalues of $\mathbf{A}$ and $\mathbf{D}$ is an orthonormal matrix, whose columns coincide with the eigenvectors of $\mathbf{A}$.

In the light of the eigendecomposition of $\mathbf{A}$ we get:

\begin{dmath}
\norm{\left( \mathbf{I} -\delta\mathbf{A}\right)^{-1} - \mathbf{S}_k} 
= \norm{\delta^k\mathbf{A}^k + \delta^{k+1}\mathbf{A}^{k+1} + \ldots} 
\leq \norm{\delta^k\mathbf{A}^k} + \norm{\delta^{k+1}\mathbf{A}^{k+1}} + \ldots = \delta^k\norm{\mathbf{A}^k} + \delta^{k+1}\norm{\mathbf{A}^{k+1}} + \ldots
\end{dmath}

\noindent
which can be further simplified by observing that, for any $j$:

\begin{dmath}
\norm{\mathbf{A}^j} = \norm{\mathbf{D}^{-1}\mathbf{\Lambda}\mathbf{D}} 
\leq \norm{\mathbf{D}^{-1}}\norm{\mathbf{\Lambda}^j}\norm{\mathbf{D}} 
= \norm{\mathbf{\Lambda}^j} 
\leq  \norm{\mathbf{\Lambda}}^j  
= \lambda_1^j
\end{dmath}

Here we used the fact that $\mathbf{D}$ and $\mathbf{D}^{-1}$ are orthonormal so their $L_2$ norm is equal to $1$. 
In addition, $\mathbf{\Lambda}$ has the same spectrum of $\mathbf{A}$ hence its $L_2$ norm coincides with the spectral radius $\lambda_1$ of $\mathbf{A}$.
By putting together the previous results we obtain:

\begin{dmath}
\norm{\left( \mathbf{I} -\delta\mathbf{A}\right)^{-1} - \mathbf{S}_k}  
\leq \delta^k\lambda_1^k + \delta^{k+1}\lambda_1^{k+1} + \ldots 
= \delta^k\lambda_1^k \left( 1 + \delta\lambda_1 + \delta^2\lambda_1^2 + \ldots\right) 
= \delta^k\lambda_1^k \frac{1}{1 - \delta\lambda_1} 
= \left(\delta \lambda_1\right)^k\frac{1}{1 - \delta\lambda_1}
\end{dmath}

\noindent
as required. 

\end{proof}

% ------------------------------------------------------------------------
\subsection{Rate of convergence for the exponential potential gain}
\label{sub:rate-convergence-exponential}

The convergence result obtained with Theorem \ref{the:convergence-geometric} above has a counterpart for the exponential potential gain. 
In Theorem \ref{the:convergence-esponential} below we give an exponential convergence result for the exponential potential gain case.


\begin{theorem}
\label{the:convergence-esponential}
Let $\G$ be a graph with adjacency matrix $\A$ and let $\lambda_1$ be the spectral radius of $\mathbf{A}$. 
If $k$ is at least $2e \lambda_1$ then 

\[
\left(\frac{1}{2}\right)^{2 e \lambda_1} \lambda_1^{-\frac{1}{2}}
\]

\noindent
is an upper bound for $\varepsilon_e(k)$. 
\end{theorem}


%----------------
\begin{proof}

Thanks to Equation \ref{eqn:exponential-potential-gain} we can define:

\[
\mathbf{S} = \sum_{i=0}^{+\infty} \frac{1}{i!} \mathbf{A}^i \quad \text{and} \quad \mathbf{S}_k = 
\sum_{i=0}^{k} \frac{1}{i!} \mathbf{A}^i
\]

\noindent
Next, we exploit the sub-multiplicativity property of the $L_2$ norm to obtain:

\begin{dmath}
\label{eq:error}
\norm{\mathbf{e} - \mathbf{e_k}} 
= \norm{\mathbf{A} \times \mathbf{S} \times \mathbf{1} - \mathbf{A} \times \mathbf{S_k}\times \mathbf{1}} 
= \norm{\mathbf{A} \times \left(\mathbf{S} -  \mathbf{S_k}\right)\times \mathbf{1}} 
\leq \norm{\mathbf{A}}\norm{\mathbf{R_k}}\norm{\mathbf{1}}
\end{dmath}

\noindent
with $\mathbf{R_k} = \mathbf{S} - \mathbf{S_k}$.
Also, by repeated application of the triangle inequality we obtain:

\begin{dmath}
\label{eqn:varepsilon}
\norm{\mathbf{R_k}} 
= \norm{\frac{\mathbf{A}^{k+1}}{\left(k+1\right)!} + \frac{\mathbf{A}^{k+2}}{\left(k+2\right)!} + \ldots}  
\leq \frac{\norm{\mathbf{A}^{k+1}}}{\left(k + 1\right)!} + \frac{\norm{\mathbf{A}^{k+2}}}{\left(k + 2\right)!} + \ldots
\end{dmath}

Recall that $\G$ is undirected so its adjacency matrix $\mathbf{A}$ is symmetric.
Thus, the $L_2$ norm of $\mathbf{A}$ coincides with its spectral radius. 
Also, for any $r \in \mathbb{N}$, $\mathbf{A}^r$ is still symmetric and, due to the sub-multiplicativity of the $L_2$ norm, we get $\norm{\mathbf{A}^r} \leq \lambda_1^r$, which allows us to simplify Equation \ref{eqn:varepsilon} as follows:



\begin{multline}
\norm{\mathbf{R_k}} \leq \frac{\lambda_1^{\left(k+1\right)}}{(k+1)!} +
\frac{\lambda_1^{\left(k+2\right)}}{(k+2)!} + \ldots =\\
= \frac{\lambda_1^{\left(k\right)}}{k!}\left[  1 + \frac{\lambda_1}{k+1} +  \frac{\lambda_1^2}{k(k+1)} +
\frac{\lambda_1^3}{k(k+1)(k+2)} + \ldots \right] \\\leq
\frac{\lambda_1^{\left( k \right)}}{k!}\left[  1 + \frac{\lambda_1}{k+1} +  \frac{\lambda_1^2}{(k+1)^2} +
\frac{\lambda_1^3}{(k+1)^3} + \ldots \right] = \\
= \frac{\lambda_1^{k}}{k!} \sum_{r=0}^{+\infty} \left(\frac{\lambda_1}{k+1}\right)^r
\end{multline}

Now, since $k + 1 > k \simeq 2e\lambda_1 > \lambda_1$, we have that $\sum_{r=0}^{+\infty} \left(\frac{\lambda_1}{k+1}\right)^r$ converges to the constant value $\frac{k+1}{k+1 - \lambda_1} \simeq \frac{2e}{2e - 1}$. 

The final step corresponds to applying Stirling's formula \cite{knuth1989concrete}, which states that, for sufficiently large values of $k$, $k! \simeq \sqrt{2\pi k} \left(\frac{k}{e}\right)^k$, which implies $k! = 2\sqrt{\pi} \lambda_1^{\frac{1}{2}} \left( 2\lambda_1\right)^{2e\lambda_1}$ if $k \simeq 2e \lambda_1$. 
Therefore, after some simplifications, we obtain

\[
\frac{\lambda_1^{k}}{k!} \simeq \frac{1}{2\sqrt{ \pi}}\left(\frac{1}{2}\right)^{2 e \lambda_1} \lambda_1^{-\frac{1}{2}}.
\]

\noindent
which completes the proof.

\end{proof}

\subsection{Computational Analysis}
\label{sub:computational}

\blue{Many previous studies focused on the problem of efficiently calculating the product $F(\mathbf{A}) \times \mathbf{b}$ where $\mathbf{A} \in \mathbb{R}^{n \times n}$, $\mathbf{b} \in \mathbb{R}^n$ and $F(\cdot)$ is an arbitrary function defined over the spectrum of $\mathbf{A}$ \cite{popolizio2008acceleration}.  \\
In many applications $\mathbf{A}$ is large and, thus, it is computationally prohibitive to first compute $F(\mathbf{A})$ and, then, to form the product $F(\mathbf{A}) \times \mathbf{b}$. \\
A clever strategy consists of projecting $\mathbf{A}$ (resp., $\mathbf{b}$) onto a matrix $\mathbf{H}$ (resp., a vector $\mathbf{w}$) of size $r\times r$ (resp., $r$) belonging to a subspace $\Omega$ such that $r$ is much smaller than $n$: in this way, we estimate the product $F(\mathbf{A}) \times \mathbf{b}$ as   
$F(\mathbf{H}) \times \mathbf{w}$ which is much easier to compute.\\
The task of projecting $\mathbf{A}$ and $\mathbf{b}$ onto $\mathbf{H}$ and $\mathbf{w}$ is equivalent to constructing an orthonormal matrix $\mathbf{V} = [\mathbf{v}_1, \mathbf{v}_2, \ldots, \mathbf{v}_r]$ whose columns span $\Omega$. 
If such a matrix $\mathbf{V}$ is available, then $\mathbf{H}$ is defined as
$\mathbf{H} = \mathbf{V}^T\mathbf{A}\mathbf{V}$ and the vector $\mathbf{b}$ is mapped onto the vector $\mathbf{w} = \mathbf{V}^T \times \mathbf{b}$.\\
The procedure for calculating $\mathbf{V}$ depends on both the spectral features of $\mathbf{A}$ as well as on the approximation accuracy we plan to obtain; in practice, the size of $\mathbf{V}$ could be very large and, thus, optimization techniques have been extensively studied to generate  good approximations of $F(\mathbf{A}) \times \mathbf{b}$.\\
One of the most popular techniques is the {\em Krylov subspace} \cite{saad1992analysis,heath2002scientific}
\begin{definition}[Standard Krylov Subspace]
Let $\mathbf{A} \in \mathbb{R}^{n \times n}$ matrix and let $\mathbf{b} \in \mathbb{R}^n$. The {\em standard Krylov subspace} of dimension $r$  associated with $\mathbf{A}$ and $\mathbf{b}$  is defined as the   
$$
\mathcal{K}_r(\mathbf{A}, \mathbf{b})=  \textsl{span} \{\mathbf{b}, \mathbf{A} \times \mathbf{b}, \ldots, \mathbf{A}^{r-1}\times \mathbf{b}\}
$$
\end{definition}
One could construct the standard Krylov subspace $\mathcal{K}_r(\mathbf{A}, \mathbf{b})$ and identify an orthonormal basis for $\mathcal{K}_r(\mathbf{A}, \mathbf{b})$; the vectors in such a basis constitute the columns of the matrix $\mathbf{V}$ we would like to compute.\\
Since $\mathbf{A}$ is symmetric the most efficient technique to find such an orthonormal basis for $\mathcal{K}_k(\mathbf{A}, \mathbf{b})$ is the {\em symmetric Lanczos algorithm} \cite{heath2002scientific}.
Such an algorithm performs $\ell$ iterations and, at each iteration, the most time-expensive step consists of calculating the product of the matrix $\mathbf{A}$ by a vector of size $n$. 
If $\mathbf{A}$ is large but sparse, the cost of each iteration is $O(n)$ and the overall cost is $O(\ell n)$ which is equal to the asymptotic cost of our algorithm.\\ 
A further, computationally-appealing option is to approximate  $F(\cdot)$ by means of a rational function $g(x)$ defined as the ratio of two polynomials, $p_{\nu}(x)$ and $q_{\mu}(x)$, of degree $\nu$ and $\mu$, respectively \cite{guttel2013rational,popolizio2008acceleration}.
In this way, the problem of calculating $F(\mathbf{A}) \times \mathbf{b}$ is equivalent to evaluate $g(\mathbf{A}) \times \mathbf{b}$ which should be hopefully easier to calculate.
If we denote as $\sigma_1, \sigma_2, \ldots \sigma_{\mu}$ the poles of $g(x)$, i.e, the roots of $q_{\mu}(x)$, then we introduce the following definition:
\\
\begin{definition}[Rational Krylov Subspace]
Let $\mathbf{A} \in \mathbb{R}^{n \times n}$ matrix and let $\mathbf{b} \in \mathbb{R}^n$. The {\em rational Krylov subspace} of dimension $r$  associated with $\mathbf{A}$ and $\mathbf{b}$  is defined as the   
$$
\mathcal{K}^{\star}(\mathbf{A}, \mathbf{b}) = \textsl{span}\{\mathbf{b}, (\mathbf{A} - \sigma_1 \mathbf{I})^{-1} \times \mathbf{b}, \ldots, (\mathbf{A} - \sigma_r \mathbf{I})^{-1} \times \mathbf{b}\}
$$
\end{definition}
Rational Krylov subspace methods are often more accurate than standard ones but they require to solve, at each iteration, a linear system; such a task is equivalent to computing terms of the form $(\mathbf{A} - \sigma_i \mathbf{I})^{-1} \times \mathbf{b}$ and such a procedure is usually much more expensive than standard Krylov methods.\\
Theorems \ref{the:convergence-geometric} and \ref{the:convergence-esponential}  indicate that our procedure is capable of achieving an exponentially decay error: consequently, we are able to achieve the accuracy we wish with a relatively small number of iterations.}





==> experiments_mod-WI19-from-TKDE-2nd-no_color.tex <==
% ------------------------------------------------------------------------
\section{Experimental validation}
\label{sec:experiments}

In this section we report on the experiments we carried out to assess the effectiveness of geometric and exponential potential gain on real-world datasets. 
Our experiments aim at answering the following questions: 
% MOD
How do the geometric and exponential potential gain correlate with other, popular, centrality metrics such as Degree, Katz and Eigenvector Centrality? \blue{Are the aforementioned centrality metrics good candidates for assessing the navigability of a node?}

% MOD
\begin{comment}
\begin{enumerate}
\item[$Q_1:$] How sensitive are our approximations of the geometric and the exponential potential gain w.r.t. the length $k$ of walks?

\item[$Q_2:$] Do our algorithms scale up to real graphs?

\item[$Q_3:$] How do the geometric and exponential potential gain correlate with other, popular, centrality metrics such as Degree, Katz and Eigenvector Centrality? \blue{Are the aforementioned centrality metrics good candidates for assessing the navigability of a node?}
\end{enumerate}
\end{comment}


To answer these questions, we considered three large, real datasets, taken from~\cite{kunegis2013konect}, whose features are described in 
Table~\ref{tbl:dataset}.
\blue{The first dataset -- \textsc{Facebook} -- is a sample of the Facebook user connections graph: in it, a node represents a Facebook user and an edge represents a friendship between two users. The second dataset, called \textsc{DBLP}, is a sample of the DBLP computer science bibliography: authors correspond to nodes and two nodes are linked by an edge if the corresponding authors have published at least one paper together. Finally, \textsc{YouTube}, is a sample of the friendship network between YouTube users.}

We implemented our algorithms in Python (with the Scipy module) on a hardware platform with the following features: AMD Ryzen 5 1600 CPU, 16GB RAM and Ubuntu 17.10.   
 
\begin{table}
\centering
\begin{tabular}{clrrrr}
\hline \hline 
& Dataset & Nodes & Edges & {$\lambda_1$} & Year\\
\hline 
1 & Facebook Friendship & $63\,731$ & $817\,035$ & $132.57$ & 2009  \\
2 & DBLP co-authorship & $317\,080$ & $1\,049\,866$ & $115.85$ &  2012 \\
3 & Youtube friendship & $1\,134\,890$ & $2\,987\,624$ & $210.40$ & 2012 \\
%4 & LiveJournal links & $5\,204\,176$ & $49\,174\,464$ \\
\hline
\end{tabular}
\caption{Key features of the datasets employed in our experimental tests. For each dataset we report the number of nodes, the number of edges, the spectral radius and the year in which data were collected.}
~\label{tbl:dataset}
\end{table}

% --------------------------------------------------------------------------------
% MOD
\begin{comment}
% --------------------------------------------------------------------------------
\subsection{The impact of walk length on the approximation of geometric/exponential potential gains}
\label{sub:accuracy-estimation}

The aim of this section is to answer question $\mathbf{Q_1}$ and, specifically, to study the quality of the approximation of the geometric and exponential potential gain in relation to walk length. 
Ideally, one would like geometric (resp., exponential) potential gain values to stabilize already for small values of $k$.
It would mean that, for any node $i$, it suffices to consider nodes located a few hops away from $i$ to get a satisfactory approximation of its geometric (resp., exponential) potential gain.

To perform our study we experimentally studied the decrease of $\varepsilon_g(k)$ and $\varepsilon_e(k)$ as function of $k$.
We start by discussing the results for the geometric potential gain, in Figures \ref{fig:error-facebook}, \ref{fig:error-dblp} and \ref{fig:error-youtube}.


\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{../img/plotGpErr_Facebook.eps}
\caption{Values of $\varepsilon_g(k)$ as a function of $k$ plotted in semi-logarithmic scale for \textsc{Facebook}}
\label{fig:error-facebook}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{../img/plotGpErr_DBLP.eps}
\caption{Values of $\varepsilon_g(k)$ as a function of $k$ plotted in semi-logarithmic scale for \textsc{DBLP}}
\label{fig:error-dblp}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{../img/plotGpErr_YouTube.eps}
\caption{Values of $\varepsilon_g(k)$ as a function of $k$ plotted in semi-logarithmic scale for \textsc{YouTube}}
\label{fig:error-youtube}
\end{figure}

A notable feature of our algorithm is that convergence is very fast, independently of the size and nature of the dataset under investigation.
For instance, with the \textsc{YouTube} dataset-- the largest tested here -- walks up to length $k = 20$ are sufficient to achieve $\varepsilon_g(k)$ lesser than $10^{-6}$.

\blue{A further observation is that, for a fixed value of $k$, the larger $\delta$, the slower the convergence of $\varepsilon_g(k)$ to zero, and that our results perfectly agree with the statement of Theorem \ref{the:convergence-geometric}.\\
It is also instructive to study how $\varepsilon_g(k)$ varies across datasets: for any value of $\delta$, $\varepsilon_g(k)$ for\textsc{DBLP} converges to zero faster than it does for \textsc{Facebook}, despite the fact that \textsc{DBLP} is about five times larger than \textsc{Facebook} (see Figures \ref{fig:error-dblp} and \ref{fig:error-youtube}).}
It is also possible to appreciate small differences in the slopes of straight lines plotting $\log \varepsilon_g(k)$ as a function of $k$.

The important finding described above is mirrored by a similar result for the exponential potential gain, as illustrated by Figure \ref{plt:errEpg}.
Once again we notice that graph size has a small impact on the convergence of our algorithm.
From Theorem \ref{the:convergence-geometric}, in fact, $\lambda_1$ is the dominant parameter: the smaller $\lambda_1$, the faster the algorithm converges to the true value of the exponential potential gain. 
Notice also how the exponential potential gain needs walks that are \textit{longer} than those needed for the geometric potential gain: we need walks up to length 169, 189 and 279 for \textsc{DBLP}, \textsc{Facebook} and \textsc{YouTube}, respectively.  

\begin{figure}[htb]
\centering
\includegraphics[width=\columnwidth]{../img/plotExpGpErr.eps}
\caption{Values of $\varepsilon_e(k)$ as a function of $k$ for the \textsc{Facebook}, \textsc{DBLP}, and \textsc{YouTube} datasets plotted in semi-logarithmic scale.}
\label{plt:errEpg}
\end{figure}

The main results of our experimental validation can be now summarized as follows: {\em (i)} For the geometric potential gain, small values of $\delta$ should be used.  Walks of length between 4 and 10 are sufficient to get a very good approximation. {\em (ii)} The time needed to compute the geometric and the exponential potential gain does not depend on the graph size but it only depends on $\lambda$: the larger $\lambda_1$ the more dense/connected the graph is and, thus, a larger number of walks is needed to achieve a good approximation. {\em (iii)} Computing the exponential potential gain is slower than computing geometric potential gain and, experimentally, it might require walks whose length is ten times larger.  This finding suggests that we should consider as future work to introduce a decay factor of the form $\frac{\delta^k}{k!}$ to penalize long walks.


% ---------------------------------------------------------------------------------
\subsection{Scalability Analysis}
\label{sub:scalability-analysis}

In this section we address question $\mathbf{Q_2}$ by studying how our algorithms scale over \textsc{Facebook}, \textsc{DBL} and \textsc{YouTube}. 
We measured the execution times as a function of the walk length $k$.
In particular, for the geometric potential gain we were concerned with understanding how $\delta$ affected the performance of our approach.
The results we obtained are plotted in Figure \ref{plt:times}.

Clearly, an increase of $\delta$ yields an increase in computational time. 
This is due to the fact that larger values of $\delta$ force our algorithm to explore the graph in more depth. 
Such effect can be clearly seen in Figure \ref{plt:times}; the increase is approximately linear in $\delta$ so we can conclude that the computational impact of increasing $\delta$ is limited.
Of course, larger datasets still require greater computational resources since we will have multiply the adjacency matrix $\mathbf{A}$ by a vector.
However, for sparse adjacency matrices the calculation is still fast, e.g., it takes less than one second for the three datasets considered here.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{../img/compTimesPg.eps}
%\includegraphics[width=0.495\columnwidth]{compTimesExpPg.eps}
\caption{Computation times vs. $\delta \lambda_1$ for the geometric potential gain}
%, Right (b): Exponential Potential Gain}
\label{plt:times}
\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.9\columnwidth]{histo_iter.eps}
%\caption{Exponential Potential Gain: number of iterations}
%\label{plt:iter_exp}
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width=0.9\columnwidth]{histo_times.eps}
%\caption{Exponential Potential Gain: Computation times}
%\label{plt:times_exp}
%\end{figure}

Table \ref{tbl:comp-times-epg} reports the computation times of the exponential potential gain. 
Again we may notice how exponential potential gain is computationally more demanding than the  geometric potential gain as we need many more iterations. 
In addition, notice how the computational time for DBLP is about three times slower than for Facebook despite the fact that the latter needed 20 iterations more.
Such difference depends on the difference in size between the two datasets.

\begin{table}[htb]
\centering
\begin{tabular}{lr}
\hline \hline 
Dataset &  Time (sec.) \\
\hline
Facebook & $0.525$ \\
DBLP &  $1.568$ \\ 
YouTube & $11.878$ \\ 
\hline \hline 
\end{tabular}
\caption{Computational times for the exponential potential gain}~\label{tbl:comp-times-epg}
\end{table}


% --------------------------------------------------------------------------------
MOD:
\end{comment}
% ----------------------------------------------------------------------------
\subsection{Relation with other centrality metrics}
\label{sub:correlation-analysis}

\blue{In this section we investigate how the geometric and the exponential potential gain are correlated with some popular centrality metrics from literature. \\ Specifically, we compared the geometric (in short {\em GPG}) and the exponential potential gain (in short {\em EPG}) with Degree Centrality ({\em DEG}), Eigenvector Centrality ({\em EC}), PageRank ({\em PR}) and Katz Centrality ({\em Katz}).
As for PageRank, we fixed the damping factor equal to $0.85$. For a fair comparison, we choose the same value of $\delta$ for {\em GPG} and {\em Katz}.\\
We applied the centrality metrics above on the \textsc{Facebook}, 
\textsc{DBLP} and \textsc{YouTube} datasets and we used the {\em Spearman's $\rho$ coefficient} to calculate the correlation between the ranked lists of nodes that each of these centrality metrics generates.\\
In Figures \ref{fig:corr-facebook-alpha}, \ref{fig:corr-dblp-alpha} and \ref{fig:corr-youtube-alpha} we plot $\rho$ as function of $\delta$.\\
From our experiments we observe that {\em GPG} and {\em Katz} have an almost perfect correlation, as one would expect: in fact, for a fixed value of $\delta$, centrality scores are highly (and positively) correlated with the geometric potential gain.
This is explained by the fact that the two coefficients differ by a multiplicative and constant factor given by the degree.
As a consequence, we may conclude that the {\em Katz} score may be interpreted as a score of navigability.}

\blue{
We note an interesting fact about the correlation of {\em GPG} and {\em EPG}. 
For Facebook (Figure \ref{fig:corr-facebook-alpha}) the $\rho$ is always above 0.8 while for \textsc{DBLP}, shown in Figure \ref{fig:corr-dblp-heatmap} it is negative, i.e., the two are inversely correlated.
Finally, for \textsc{YouTube}, the $\rho$  decreases from -0.75 to -1 as $\delta$ grows.
To explain the differences emerging across our datasets we observe that the eigenvalues $\lambda_i$ of $\G$ are transformed into $\lambda_i^{\prime} = \frac{\lambda_i}{1-\lambda_i}$ in case of {\em GPG} and into $\lambda_i^{\prime\prime} = \lambda_i e^{\lambda_i}$ in case of EPG (see Equation \ref{eqn:lambda_gpg} and \ref{eqn:lambda_epg}). 
The difference $\lambda_i^{\prime} - \lambda_i^{\prime\prime}$ is related, by Equation \ref{eqn:difference-geometric-potential}, to the observed difference between the {\em GPG} and {\em EPG}. 
Therefore, on the basis of the distribution of eigenvalues, we conclude that for some datasets {\em GPG} and {\em EPG} might be strongly and positively correlated while they are negatively correlated elsewhere.}

\blue{
Consider now Degree Centrality.
An increase in $\delta$ generally causes a decrease in $\rho$, with the exception of the \textsc{DBLP} dataset where the correlation between {\em DEG} and {\em GPG} is almost perfect. 
Observe that, if $\delta \to 0$, then the {\em GPG} is well approximated by {\em DEG}, by definition. 
Vice versa, as $\delta$ gets larger walks of length greater than one  increasingly contribute to the geometric potential gain, thus amplifying the difference between Degree Centrality and the geometric potential gain.
\\
As it can be seen from Figures \ref{fig:corr-facebook-heatmap}, \ref{fig:corr-dblp-heatmap} and \ref{fig:corr-youtube-hatmap}, {\em DEG} and {\em GPG} are highly and positively correlated ($\rho \in [0.84, 1]$) and this to some extent explains the correlation between {\em GPG} and {\em PR} (even though we are aware of high correlation between Katz and PageRank).\\
Let us now consider the correlation between {\em EC} and {\em GPG}: when $\delta$ increases the two metrics tend to become more and more correlated.
However, while for \textsc{Facebook} such correlation is positive and converges to $1$ for \textsc{YouTube} and \textsc{DBLP} it is negative and tends to $-1$ (for increasing values of $\delta$). 
Such behaviour clearly depends on the fact that $\delta$ can be at most $\frac{1}{\lambda_1}$. 
For values of $\delta$ approaching $\frac{1}{\lambda_1}$, Katz and Eigenvector centrality become almost equal.
This ultimately implies that the {\em GPG} and {\em EC} differ by a constant factor and thus appear to be strongly related.}



\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{../img/facebook-centrality-scores-correlation.png}
\caption{Spearman's $\rho$ correlation between Geometric Potential Gain and DEG, EC, PR, Katz as function of $\delta$ on the \textsc{Facebook} dataset. }
\label{fig:corr-facebook-alpha}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{../img/heatmap-FB-trimmed.png}
\caption{Spearman's $\rho$ correlation between DEG, EC and PR on the \textsc{Facebook} dataset. }
\label{fig:corr-facebook-heatmap}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{../img/dblp-centrality-scores-correlation.png}
\caption{Spearman's $\rho$ correlation between Geometric Potential Gain and DEG, EC, PR, Katz as function of $\delta$ on the \textsc{DBLP} dataset.}
\label{fig:corr-dblp-alpha}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{../img/heatmap-DBLP-trimmed.png}
\caption{Spearman's $\rho$ correlation between DEG, EC and PR on the \textsc{DBLP} dataset. }
\label{fig:corr-dblp-heatmap}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{../img/youtube-centrality-scores-correlation.png}
\caption{Spearman's $\rho$ correlation between Geometric Potential Gain and DEG, EC, PR, Katz as function of $\delta$ on the \textsc{YouTube} dataset. }
\label{fig:corr-youtube-alpha}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{../img/heatmap-YT-trimmed.png}
\caption{Spearman's $\rho$ correlation between DEG, EC and PR on the \textsc{YouTube} dataset. }
\label{fig:corr-youtube-hatmap}
\end{figure}



%\begin{figure}[!t]
%\centering
%\includegraphics[width=\columnwidth]{../img/correlation_scores_FB-tight.png}
%\caption{Correlation between the geometric and the exponential potential gain with Degree Centrality and Katz Centrality scores for the  \textsc{Facebook} dataset. In the figure $PG(0.15)$, $PG(0.43)$, $PG(0.72)$ and $PG(1)$ specify the geometric potential gain for $\delta = 0.15\lambda_1^{-1}$, $\delta = 0.43\lambda_1^{-1}$, $\delta = 0.72\lambda_1^{-1}$ and $\delta = 1\lambda_1^{-1}$, respectively. Analogously, $K(0.15)$, $K(0.43)$, $K(0.72)$ specifies the Katz Centrality score for $\delta = 0.15\lambda_1^{-1}$, $\delta = 0.43\lambda_1^{-1}$, $\delta = 0.72\lambda_1^{-1}$, respectively. Finally $K(1)$ is the Eigenvector Centrality.}
%\label{fig:corr-facebook}
%\end{figure}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=\columnwidth]{../img/correlation_scores_DBLP-tight.png}
%\caption{Correlation between the geometric and the exponential potential gain with Degree Centrality and Katz Centrality scores for the  \textsc{DBLP} dataset. In the figure $PG(0.15)$, $PG(0.43)$, $PG(0.72)$ and $PG(1)$ specify the geometric potential gain for $\delta = 0.15\lambda_1^{-1}$, $\delta = 0.43\lambda_1^{-1}$, $\delta = 0.72\lambda_1^{-1}$ and $\delta = 1\lambda_1^{-1}$, respectively. Analogously, $K(0.15)$, $K(0.43)$, $K(0.72)$ specifies the Katz Centrality score for $\delta = 0.15\lambda_1^{-1}$, $\delta = 0.43\lambda_1^{-1}$, $\delta = 0.72\lambda_1^{-1}$, respectively. Finally $K(1)$ is the Eigenvector Centrality.}
%\label{fig:corr-dblp}
%\end{figure}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=\columnwidth]{../img/correlation_scores_YT-tight.png}
%\caption{Correlation between the geometric and the exponential potential gain with Degree Centrality and Katz Centrality scores for the  \textsc{YouTube} dataset. In the figure $PG(0.15)$, $PG(0.43)$, $PG(0.72)$ and $PG(1)$ specify the geometric potential gain for $\delta = 0.15\lambda_1^{-1}$, $\delta = 0.43\lambda_1^{-1}$, $\delta = 0.72\lambda_1^{-1}$ and $\delta = 1\lambda_1^{-1}$, respectively. Analogously, $K(0.15)$, $K(0.43)$, $K(0.72)$ specifies the Katz Centrality score for $\delta = 0.15\lambda_1^{-1}$, $\delta = 0.43\lambda_1^{-1}$, $\delta = 0.72\lambda_1^{-1}$, respectively. Finally $K(1)$ is the Eigenvector Centrality.}
%\label{fig:corr-youtube}
%\end{figure}


%With Katz's centrality, as one would expect, for a fixed value of $\delta$, centrality scores are highly (and positively) correlated with the geometric potential gain.
%This is explained by the fact that the two coefficients differ by a multiplicative and constant factor given by $\mathbf{A}$.

%An interesting relationship emerges between Eigenvector Centrality and the geometric potential gain: when $\delta$ increases the two metrics tend to become more and more correlated.
%However, while for Facebook such correlation is positive and converges to $1$ for YouTube and DBLP it is negative and tends to $-1$ (for increasing values of $\delta$). 
%Such behaviour clearly depends on the fact that $\delta$ can be at most $\frac{1}{\lambda_1}$. 
%For values of $\delta$ approaching $\frac{1}{\lambda_1}$ Katz and Eigenvector centrality become almost equal.
%This ultimately implies that geometric potential gain and eigenvector centrality differ by a constant factor and thus appear to be strongly related.  
%
%
% ------------- END OF VISIBLE PART -----------------------------------------
%
%
%
%To gain an understanding of why $\rho$ depends on $\delta$, let us fix $\delta$ as large as possible; in this case, \lq\lq long walks\rq\rq are effective in calculating geometric potential gain and let $\mathcal{W}(\delta)$ be the set of walks employed to calculate geometric potential gain.
%Of course, a node $i$ which displays a \lq\lq large\rq\rq geometric potential gain is traversed by many of the walks in $\mathcal{W}$; if we uniformly sample walks from $\mathcal{W}$, then a sampled walk displays a large probability of visiting that node and such a probability, by definition, coincides with the Eigenvector Centrality of $i$.
%If $delta$ decreases, then the size of $\mathcal{W}(\delta)$ decreases to and this implies a decrease in the Geometric Potential Gain of a node, while its eigenvector Centrality remains fixed. 


%A further test was performed in order to determine the 
%correlation among centrality metrics. 
%%
%We calculated the degree distribution, the Katz centrality score (for three different values of alpha) 
%distribution and the Potential Gain (for the same values of alpha  used in the Katz centrality score). 
%%
%Results are reported in the four plots reported in Figure~\ref{plt:corr}. 
%%
%We notice that for small values of alpha, Degree, PG scores and Katz scores were highly correlated 
%and this is not surprising: for instance, if we set alpha = 0, PG scores and Degree exactly coincide. 
%This result is consistent with the theoretical results discussed in the previous 
%section. 
%%
%If alpha increases, the contribution of paths in the graph G of length longer than 2 gets more and more 
%important and this leads to relevant differences in Degree, PG and Katz scores. 
%%
%This explains why we find out smaller values of correlation. 
%

%\begin{figure}
%\centering
%\includegraphics[width=0.495\columnwidth]{correlation_scores_Facebook.eps}
%\includegraphics[width=0.495\columnwidth]{correlation_scores_DBLP.eps}
%\includegraphics[width=0.495\columnwidth]{correlation_scores_YouTube.eps}
%\includegraphics[width=0.495\columnwidth]{correlation_scores_Livejournal.eps}
%\caption{Correlation between Potential Gain and some other centrality metrics. Top-Left: Facebook, Top-Right: DBLP, 
%Bottom-Left: YouTube, Bottom-Right: Livejournal}
%\label{plt:corr}
%\end{figure}

%% OLD STUFF %%
\iffalse

\textcolor{blue}{Here we need to be clear what the objective of the experimentation is.
\renewcommand{\labelenumi}{(\roman{enumi})}
\begin{enumerate}
\item We may claim that our algorithms lead to more efficient implementation of eigenvector centrality on large social networks.
\item We may claim, that in some well-defined sense our algorithms lead to ``better searchability'' in social networks.
\item We may claim that our algorithms lead to more robust networks, in some well-defined sense. This could be the topic of a followup paper. !!
\end{enumerate}
}

\fi


\iffalse
\begin{figure}[htb]
\centering
\includegraphics[width=0.9\columnwidth]{../plotGpErr_DBLP.eps}
\caption{PG: \err{} vs number of iteration for different values of delta. Data set: DBLP}
\label{plt:errDBLP}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\columnwidth]{../plotGpErr_YouTube.eps}
\caption{PG: \err{} vs number of iteration for different values of delta. Data set: YouTube}
\label{plt:errYT}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\columnwidth]{../plotGpErr_Livejournal.eps}
\caption{PG: \err{} vs number of iteration for different values of delta. Data set: Livejournal}
\label{plt:errLJ}
\end{figure}


\begin{figure}[htb]
\centering
\includegraphics[width=0.9\columnwidth]{../plotExpGpErr_DBLP.eps}
\caption{Exponential PG: \err{} vs number of iteration for different values of delta. Data set: DBLP}
\label{plt:errEpgDBLP}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\columnwidth]{../plotExpGpErr_YouTube.eps}
\caption{Exponential PG: \err{}  vs number of iteration for different values of delta. Data set: YouTube}
\label{plt:errEpgYT}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\columnwidth]{../plotExpGpErr_Livejournal.eps}
\caption{Exponential PG: \err vs number of iteration for different values of delta. Data set: Livejournal}
\label{plt:errEpgLJ}
\end{figure}


\begin{figure}[htb]
\centering
\includegraphics[width=0.9\columnwidth]{../correlation_scores_DBLP.pdf}
\caption{Correlation. Data set: DBLP}
\label{plt:corrDBLP}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\columnwidth]{../correlation_scores_YouTube.pdf}
\caption{Correlation. Data set: YouTube}
\label{plt:corrYT}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\columnwidth]{../correlation_scores_Livejournal.pdf}
\caption{Correlation. Data set: Livejournal}
\label{plt:corrLJ}
\end{figure}
\fi


==> related-works.tex <==
% --------------------------------------------------
\section{\red{Related Work}}
\label{sec:related-works}

The task of searching for and navigating in large networks has been extensively studied in the past for a broad range of domains such as routing in small world networks \cite{travers1967small}, locating pages in the World Wide Web \cite{menczer2002growing,broder2000graph}, finding the most knowledgeable individual in an enterprise/academic social network, discovering resources in a P2P network and building recommender systems \cite{lamprecht2016method}. 
Inspired by the classification scheme introduced by Helic {\em et al.}, \cite{helic2013models}, we divide search and navigation into two main classes: {\em (a) Endogenous Search}. 
In this class, there are {\em multiple} agents embedded in the network and the navigation task is depicted as a decentralized decision process in which agents collaborate to discover a path in the network.
Agents are assumed to have only a local knowledge of the network topology and, in addition, querying a neighboring node (e.g., to route a message) may have a non-negligible cost. {\em (b) Exogenous Search}. 
This class occurs whenever a user aims at navigating the Web \cite{fenner2008modelling,levene2004navigating} or an information network \red{such as} Wikipedia \cite{west2012automatic,lamprecht2017structure}. 
In exogenous search, there is {\em only one} agent involved in navigation task and it does not belong to the network. 
As in endogenous search, the agent (either human and artificial) only posses local knowledge about the network topology.
Hence, an agent has to rely on its intuition to select the next node to visit. 
Unlike the endogenous search, however, the cost for visiting a node is generally low.

In the following two sections we review methods in endogenous and exogenous search (see Sections \ref{sub:endogenous-search} and \ref{sub:exogenous-search} \red{below}).

% -------------------------------------------------------------
\subsection{Endogenous search approaches}
\label{sub:endogenous-search}

%As described earlier, one of the first \red{experiments} investigating search in \red{social networks} is due to Travers and Milgram \cite{travers1967small}, who studied connectivity patterns in a graph mapping \lq\lq who-knows-whom\rq\rq relationships between people in the United States. 
%Their experiment demonstrated two surprising facts about real social networks: firstly, social networks contain a wealth of short paths and, secondly, ordinary people are able to detect them rather quickly, even if they act without the support of a ``global map'' depicting the network of human contacts.

Many mathematical models have been proposed to explain why networks are, in an informal sense, \textit{navigable.}
Some of the best-known models are described in \cite{kleinberg2000navigation,kleinberg2000small,kleinberg2002small,watts2002identity}.
The original Watts-Strogatz (WS) model \cite{watts1998collective} generated random graphs in which pairs of nodes belonging to distant parts of the graph may be connected through random edges, called {\em long-range weak ties.} 
The WS model was thus effective in forcing the graph to be ``small,'' i.e., to assure the presence of paths consisting of few edges between any pair of nodes. 
Nevertheless, the WS model alone is unable to explain why people are capable of discovering such paths.
%The main shortcoming in the WS model is that it ignored the influence of homophyly in social links: nodes of social networks may share some features (e.g., age, job, location) that facilitate the emergence of social links. 
%In the WS model, long-range weak ties are totally independent of node similarity and, therefore, it is unable to reproduce homophyly-based social ties.

A first class of approaches to search large network relies on the notion of {\em popularity} and the approach of Adamic et al. \cite{adamic2001search} is perhaps the best-known approach in that category: here the search task is modelled as a random walk on the graph $\G$. In a specific step, if the walker occupies a node $l$ which is not
the target one (and none of the neighbours of $l$ is the target one), then the walker chooses the unvisited neighbour with largest degree. Such a strategy achieves significant computational savings, especially if $\G$ follows a power-law topology.

Another class of approaches -- called {\em similarity-based approaches} -- exploit homophily to speed up search tasks \cite{kleinberg2000small,watts2002identity}.
Kleinberg \cite{kleinberg2000navigation} described a generalization of the WS model to explain why decentralized search is effective in real networks. 
In Kleinberg's model, nodes of a social network are arranged to form a bi-dimensional grid (called {\em a lattice);} each node is connected to its neighbours in the lattice and, in particular, the distance $d(u, v)$ between two nodes equals the number of grid steps separating them. 
As a result, each node $v$ is connected to its \red{four} local contacts (i.e., nodes at distance one from $v$).
In addition, a random edge---called {\em long range edge}---connecting $v$ with a node $k$ is generated with probability proportional to $d(v,k)^{-q}$, $q$ being the so-called clustering exponent of the model.
Kleinberg proved that if $q = 2$, then the performance of decentralized search is optimal, i.e. there exists an algorithm that, on average, is able to deliver a message from an arbitrary source node to an arbitrary target in $O(\log^2 n)$ time. 

Another contribution is due to Watts {\em et al.} \cite{watts2002identity} who proposed a model to explain network navigability in which nodes aggregate into {\em groups} on the basis of some shared attributes such as job or geographic location. 
For each attribute, a population can be split into a hierarchical set of layers $\mathcal{H}$ in which the top layer describes the entire population, while layers at increasing depth define a cognitive division of the population into more specific groups. 
Individuals can manage two kinds of information to decide to whom a message should be forwarded to:  first, {\em social distance}, which accounts for the similarity of two nodes and, second, {\em network distance}, i.e., the number of network paths that can be detected by looking at the neighbors. 

Social distance between two individuals $i$ and $j$ can be estimated by considering the groups $i$ and $j$ belong to and how distant these groups are in the layers of $\mathcal{H}$. 
As such, social distance is a kind of global metrics but, unfortunately, it is not a true distance in the sense that individuals belonging to close groups may be separated by long paths in the social network graph. 

Network distance, on the other hand, is a true distance but a node only has access to a local portion of the network and, thus, it can correctly calculate network distances only for nodes which are separated from it by  few hops.
By means of simulations \cite{watts2002identity} proved that social distance is effective in approximating network distance and, thus, to successfully in directing messages across the network.

More recently Csimcsek {\em et al.} \cite{csimcsek2008navigating} suggest to combine popularity- and similarity-based methods and, to this end, they describe a graph search algorithm that, at each step, forwards a message from the current node $i$ to one of its neighbours, say $j$, such that the product $d_i \times q_{ij}$ is maximum; here $q_{ij}$ quantifies homophily between $i$ and $j$.

\blue{Unlike the approaches above, which assume that some attributes are available at each node, our approach only makes use of connectivity patterns to calculate the centrality of a node.}


% -------------------------------------------------------------------
\subsection{Exogenous search approaches}
\label{sub:exogenous-search}

Exogenous search is mostly related to search in information networks such as a collection of Web pages or Wikipedia. 



One of the most common search strategies on the World Wide Web (WWW) is {\em surfing}, in which a user moves from a Web page to another one by following hyperlinks. 
Huberman {\em et al.} \cite{huberman1998strong} introduced a probabilistic model to describe surfing. 
In this model, the sequence of Web pages a user visits is regarded as the realisation of a random process and each Web page is associated with a value to the user. 
A user will stop surfing if the estimated cost of accessing a new Web page is bigger than the expected value of the information the user may get from accessing it. 

More recently, West and Leskovec \cite{west2012human} analysed how people navigate an information network such as Wikipedia in order to reach a specific target. 
To this end, they used an online computation game, called {\em Wikispeedia} \cite{west2009wikispeedia}, in which Wikipedia information seekers are given two random articles and they are required to navigate from one to the other by clicking as few hyperlinks as possible. 
In a subsequent paper \cite{west2012automatic}, they compared the accuracy of several decentralized search algorithms and benchmarked them  against  the  human  navigation  paths.  
Such a study highlighted two main phases of human navigation in information networks: 
{\em (i) Zoom-Out}: here, users strives to reach the network {\em core} (or a hub in the network core); such a core consists of a Wikipedia page with many links to other pages in Wikipedia. 
In this step, humans would prefer pages with many outgoing links ({\em high degree pages}). 
{\em (ii)  Zoom-in}, in  which  users leave the core to get closer to a topic. Specifically, if we think of segmenting Wikipedia pages into clusters on the basis of their topics, such a phase would consist of entering into a cluster. In the zoom-in phase, users prefer to look for similar nodes in order to orient their search.

A nice approach to combine decentralized search was described by Helic {\em et al.} \cite{helic2013models} who applied decentralized search algorithms such as those described in \cite{kleinberg2000navigation} to model human navigation in information networks. 
They considered an online navigation game (called {\em WikiGame}); in this game, a user starts from a random Wikipedia page and navigates to a target page.
More than 250,000 click paths were collected  and studied to determine the factors influencing players' decisions. 
The main finding in \cite{helic2013models} is that two mechanisms regulate the way humans seek for information in large networks: i) {\em exploitation,} i.e., humans follow specific hyperlinks whenever they are confident enough that those will get them closer to the target they want, and ii) {\em exploration}, i.e., users navigate at random an information network, when their knowledge about how current links relates to a target Web page is insufficient. 
The quantitative analysis showed that exploration steps account, on average, for $15-20\%$ of collected links, while exploitation accounted for the remaining $80-85\%$ of collected links.

